UniRAG: Universal Retrieval Augmentation for Large Vision Language Models

Recently, Large Vision Language Models (LVLMs) have unlocked many complex use cases that require Multi-Modal (MM) understanding (e.g., image captioning or visual question answering) and MM generation (e.g., text-guided image generation or editing) capabilities. To further improve the output fidelityof LVLMs we introduce UniRAG, a plug-and-play technique that adds relevant retrieved information to prompts as few-shot examples during inference. Unlike the common belief that Retrieval Augmentation (RA) mainly improves generation or understanding of uncommon entities, our evaluation results on the MSCOCO dataset with common entities show that both proprietary models like GPT-4o and Gemini-Pro and smaller open-source models like LLaVA, LaVIT, and Emu2 significantly enhance their generation quality when their input prompts are augmented with relevant information retrieved by Vision-Language (VL) retrievers like UniIR models. All the necessary code to reproduce our results is available at https://github.com/castorini/UniRAG

==> figures/emu2_visualization.tex <==
\begin{figure*}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc|cc}
\subfloat[$k=0$ Emu2-G]{\includegraphics[width=0.21\textwidth]{demo_images/emu2.jpg}} &
\subfloat[$k=1$ CLIP-SF]{\includegraphics[width=0.21\textwidth]{demo_images/clip.jpg}} &
\subfloat[$k=1$ Emu2-G]{\includegraphics[width=0.21\textwidth]{demo_images/emu2_clip.jpg}} &
\subfloat[$k=1$ BLIP-FF]{\includegraphics[width=0.21\textwidth]{demo_images/blip.jpg}} &
\subfloat[$k=1$ Emu2]{\includegraphics[width=0.21\textwidth]{demo_images/emu2_blip.jpg}}\\

\end{tabular}%
}
\caption{Image generation with Emu2-Gen for \textit{``Wooden spoons and forks are all over a table."}. (a) shows zero-shot generation, (b)/(d) show top retrieved candidate from CLIP-SF/BLIP-FF, and (c)/(e) show one-shot generation using retrieved candidates as in-context examples.}
\label{fig:emu2-visual}
\end{figure*}

==> figures/figure_image_generation_few_shot.tex <==
\begin{figure}[!tbh]
\tiny
\justifying
\begin{minted}[fontsize=\tiny, frame=lines, frame=single,linenos=false,breaklines,breaksymbol=,escapeinside=||,bgcolor=LightGray]{text}
You are an intelligent assistant that can comprehend images based on their relevance to a provided caption.
I have provided you with {num} sample images.
You have to generate an appropriate image for the given __caption__ based on the provided sample images, logical reasoning, internal knowledge and common sense.
The generated image should be the best representation of all the details and descriptions in the provided caption.

__caption__: {caption}

Only respond with the image, do not say any word or explain.
\end{minted}
\vspace*{-0.5cm}
\caption{Few-shot prompting for image generation.}
\label{fig:few-shot-prompt-img}
\end{figure}

==> figures/image_caption_visualization.tex <==
\begin{figure*}
\centering
\begin{tabular}{c c |l}
\toprule
\toprule
 &  & \multicolumn{1}{c}{\includegraphics[width=0.4\textwidth]{demo_images_emnlp/COCO_val2014_000000559665.jpg}}\\
 \midrule
 \midrule
 \multirow{2}{*}{\rotatebox[origin=c]{90}
 {\text{\footnotesize\textbf{Prompt}}}} & $k=0$  & Instruction + Query image\\
 & $k=1$  & Instruction + Retrieved image-caption pair + Query image\\
 \midrule
 \midrule
 \multirow{2}{*}{\rotatebox[origin=c]{90}
 {\text{\footnotesize\textbf{LLaVA}}}} & $k=0$  & A yellow fire hydrant with a red top.\\
 & $k=1$  & A fire hydrant with a neon blue glow pouring water.\\
 \midrule
  \multirow{4}{*}{\rotatebox[origin=c]{90}
 {\text{\footnotesize\textbf{GPT-4o}}}} & $k=0$  & A long exposure photograph capturing the light trails of a passing vehicle on a \\ && quiet street at night, with a yellow fire hydrant in the foreground.\\
 & $k=1$  & A fire hydrant at night releasing a stream of water illuminated with a striking \\& & neon blue light.\\
 \midrule
  \multirow{4}{*}{\rotatebox[origin=c]{90}
 {\text{\footnotesize\textbf{Gemini-Pro}}}} & $k=0$  & A long exposure photograph of a fire hydrant at night with blue and white light \\ && trails in the background.\\
 & $k=1$  & A fire hydrant spewing out streams of blue water at night, looks like a scene from \\ && a movie with its almost surreal appearance.\\
\bottomrule
\end{tabular}

\caption{Image captioning results using CLIP-SF as retriever. The figure showcases caption examples for $k \in \{0, 1\}$ for LLaVA, GPT-4o and Gemini-Pro. Please refer Appendix~\ref{sec:prompt-details} for more details about the prompt. Figure~\ref{fig:caption-retriever} presents the retrieved query-image pair for the query image.}
\label{fig:image-cap-visual}
\end{figure*}

==> figures/image_captioning_retriever.tex <==
\begin{table*}[thb]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c | p{3cm} | p{3cm} p{3cm} p{3cm}}
\toprule
&
\centering \textbf{Query Image} &
\multicolumn{3}{c}{\textbf{Retrievered image-caption pair $k=1$}}\\
&
\centering Zero-shot &
\centering CLIP-SF &
\centering BLIP-FF &
\centering\arraybackslash Random\\
\midrule
\multirow{2}{*}{Prompt} &
\centering \includegraphics[align=b,width=0.18\textwidth]{demo_images_emnlp/COCO_val2014_000000559665.jpg}
&
\centering \includegraphics[align=b,width=0.18\textwidth]{demo_images_emnlp/500.jpg}
&
\centering \includegraphics[align=b,width=0.18\textwidth]{demo_images_emnlp/COCO_val2014_000000562592.jpg}
&
\centering\arraybackslash \includegraphics[align=b,width=0.18\textwidth]{demo_images_emnlp/COCO_val2014_000000221700.jpg}
\\
\cmidrule{2-5}
&
\centering -&
Black and white photograph of two men on motorcycles. &
A man riding on the back of a motorcycle down a highway. &
A pair of red scissors sitting on a newspaper. \\
\midrule
\midrule
LLaVA &
Motorcycle rider on the road, with luggage attached to the back.&
Black and white photograph of a man on a motorcycle.&
A man riding on the back of a motorcycle down a highway.&
A man is sitting on a motorcycle, and there are two and a half hotdogs on paper plates on a counter.\\
\midrule
Gemini-P &
&
Black and white photograph of a man and woman riding on a motorcycle.&
Two people riding on a motorcycle through a parking lot.&
Biker and his passenger riding down the road.\\
\midrule
GPT-4 &
two people on a motorcycle waiting at a traffic light.&
black and white photograph of two men on a motorcycle at an intersection.&
two people riding on a motorcycle through an intersection.&
two people are sharing a large cruiser motorcycle at a stoplight.\\
\bottomrule
\end{tabular}%
}
\caption{}
\label{tab:caption-retriever}
\end{table*}


==> figures/lavit_visualization.tex <==
\begin{figure*}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc|cc}
\subfloat[$k=0$ LaVIT]{\includegraphics[width=0.21\textwidth]{demo_images/lavit.jpg}} &
\subfloat[$k=1$ CLIP-SF]{\includegraphics[width=0.21\textwidth]{demo_images/clip.jpg}} &
\subfloat[$k=1$ LaVIT]{\includegraphics[width=0.21\textwidth]{demo_images/lavit_clip.jpg}} &
\subfloat[$k=1$ BLIP-FF]{\includegraphics[width=0.21\textwidth]{demo_images/blip.jpg}} &
\subfloat[$k=1$ LaVIT]{\includegraphics[width=0.21\textwidth]{demo_images/lavit_blip.jpg}}\\

\end{tabular}%
}
\caption{Image generation with LaVIT for \textit{``Wooden spoons and forks are all over a table."}. (a) shows zero-shot generation, (b)/(d) show top retrieved candidate from CLIP-SF/BLIP-FF, and (c)/(e) show one-shot generation using retrieved candidates as in-context examples.}
\label{fig:lavit-visual}
\end{figure*}

==> tables/caption_modality_analysis.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lc|cccc}
\toprule
\toprule
          & $k=1$ & $k=2$  & $k=3$  & $k=4$ & $k=5$          \\
\midrule
\midrule
CLIP-SF  & 4989 & 4996 & 4995 & 4995 & 4990 \\

\midrule
BLIP-FF  & 3982 & 4364 & 4527 & 4600 & 4600 \\

\bottomrule
\end{tabular}
\caption{The number of retrieved candidates with text modality in each retrieval index for CLIP-SF and BLIP-FF. 5k images from the M-BEIR's MSCOCO image-to-text test set are used as the query pool.}

\label{tab:caption-modality-analysis}
\end{table}


==> tables/image_modality_analysis.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lc|cccc}
\toprule
\toprule
          & $k=1$ & $k=2$  & $k=3$  & $k=4$ & $k=5$          \\
\midrule
\midrule
CLIP-SF  & 4629 & 4658 & 4838 & 4884 & 4892  \\

\midrule
BLIP-FF  & 3769 & 4041 & 4464  & 4623 & 4727  \\

\bottomrule
\end{tabular}
\caption{The number of retrieved candidates with image modality in each retrieval index for CLIP-SF and BLIP-FF. 5k captions sampled from the M-BEIR's MSCOCO text-to-image test set are used as the query pool.}
\label{tab:image-modality-analysis}
\end{table}

